The Uncanny Similarity of Recurrence and Depth

It is widely believed that deep neural networks contain layer specialization, wherein neural networks extract hierarchical features representing edges and patterns in shallow layers and complete objects in deeper layers. Unlike common feed-forward models that have distinct filters at each layer, recurrent networks reuse the same parameters at various depths. In this work, we observe that recurrent models exhibit the same hierarchical behaviors and the same performance benefits with depth as feed-forward networks despite reusing the same filters at every recurrence. By training models of various feed-forward and recurrent architectures on several datasets for image classification as well as maze solving, we show that recurrent networks have the ability to closely emulate the behavior of non-recurrent deep models, often doing so with far fewer parameters.

==> app_arxiv.tex <==
\section{Appendix}
\label{sec:app}

\subsection{Model Architectures}
\label{sec:app_architectures}

We train and test MLPs, ConvNets, and residual networks on three image classification datasets. These models are described in Section \ref{sec:architectures}, but the specific widths used for each dataset are detailed below.

\par \textbf{Multi-Layer Perceptrons (MLPs).} All of the MLPs have a single fully connected layer before the internal module, and a single fully connected layer afterward. Each layer in an MLP can be defined by a matrix dimension. See Table \ref{tab:mlp_archs}.

\begin{table}[h]
    \centering
    \caption{MLPs: The size of each fully connected layer in the MLPs we use for image classification.}
    \label{tab:mlp_archs}
    \begin{tabular}{lccc}
    \toprule
    % \multicolumn{4}{c}{MLPs} \\
    Dataset & First Layer & Internal Layers & Last Layer \\
    \hline
    CIFAR-10 &  $3072 \times 200$ & $200 \times 200$ & $200 \times 10$ \\
    SVHN &  $3072 \times 500$ & $500 \times 500$ & $500 \times 10$ \\
    EMNIST &  $3072 \times 500$ & $500 \times 500$ & $500 \times 47$ \\
    \bottomrule
    \end{tabular}
\end{table}

\par \textbf{ConvNets.} The ConvNets have two convolutional layers before the internal module and one convolutional and one fully connected layer afterward. Each convolutional layer is followed by a ReLU activation, and there are pooling layers before and after the last convolutional layer. For all convolutional layers outside of the internal module, we use $3 \times 3$ filters with stride of 1 and no padding. In order to preserve the exact shape of the inputs, the internal module has convolutional layers with $3 \times 3$ kernels, a stride of one pixel, and padding of one pixel in each direction.

\begin{table}[h!]
    \centering
    \caption{ConvNets: The number of channels in the output of each layer.}
    \label{tab:cnn_archs}
    \begin{tabular}{lccccc}
    \toprule
    % \multicolumn{6}{c}{ConvNets} \\ 
    Dataset &  First Layer & Second Layer & Internal Layers & Last Conv Layer & Linear Layer \\
    \hline
    CIFAR-10 & 32 & 64 & 64 & 128 & 10 \\
    SVHN & 32 & 64 & 64 & 128 & 10 \\
    EMNIST & 32 & 64 & 64 & 128 & 47 \\
    \bottomrule
    \end{tabular}
\end{table}
    

\par \textbf{Residual Networks.} The residual networks employ convolutional layers with $3 \times 3$ kernels. The first layer has a stride of two pixels and padding of one pixel in every direction. Each layer in the internal modules has striding by one pixel, while the final convolutional layer strides by two pixels. There are ReLU activations after every convolution, and average pooling before the linear layer. All the convolutional layers output 512 channels.
% \begin{table}[h!]
%     \vspace{-10pt}
%     \centering
%     \caption{Residual Networks: The number of channels in the output of each layer.}
%     \label{tab:resnet_archs}
%     \vspace{5pt}
%     \begin{tabular}{lcccc}
%     \toprule
%     % \multicolumn{5}{c}{Residual Networks} \\ 
%     Dataset &  First Layer & Internal Layers & Last Conv Layer & Linear Layer \\
%     \hline
%     CIFAR-10 & 512 & 512 & 512 & 10 \\
%     SVHN & 512 & 512 & 512 & 10 \\
%     EMNIST & 512 & 512 & 512 & 47 \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:arch_details_rescl}
% \end{table}

We also train and test residual networks with BatchNorm in order to compare the performance with ResNet-18 models. These residual networks have a unique batch norm layer after every convolutional layer followed by ReLU activation function. Since the input to the internal module at iteration $n$ is the output at iteration $n-1$ (for $n=2,3,4,...$), the batch statistics for every iteration is different. Thus, we use separate batch norm layer for each iteration.


\textbf{Maze Solvers.} For solving mazes, we train and test residual networks with slightly different architectures. These models are fully convolutional and every convolutional layer has $3 \times 3$ kernels that stride by one pixel with padding of one pixel in each direction. They have one layer before the internal module, residual blocks of four layers in the internal module, and three convolutional layers afterward. All of the layers before the third to last one have 128 output channels, and in the final three layers the numbers of output channels are 32, 8, and 2.


\subsection{Hyperparameters}
\label{sec:app_hyperparams}
All the models are trained to convergence using suitable hyperparameters. For each model and each dataset, we fine tune the number of epochs, along with the learning rate and the decay schedule. For specifics, see the launch files in the code repository at \url{https://github.com/Arjung27/DeepThinking}.

\subsection{Compute Resources}
\label{sec:app_compute}

All of our experiments are done on Nvidia GeForce RTX 2080Ti GPUs. All training, except for ImageNet models, is done on a single GPU. We train models on ImageNet data using four GPUs at a time.  Each image classification model can be trained in several hours on a single GPU, and maze solving models require eight hours. 

\subsection{Additional Visualizations}
\label{sec:app_vis}

The discussion about activation patterns in  Section \ref{sec:feature_reuse} continues here with depictions of the activity in a ConvNet trained on SVHN and a residual network trained on CIFAR-10. See Figures \ref{fig:activations_svhn} and \ref{fig:activations_resnet}. Although these plots show distinct behavior from Figure \ref{fig:activations} in the body of this paper, the conclusions are consistent. In recurrent models, features are being reused. This is clear since every filter is being used on more than one iteration, and for many filters there is significant activity in most iterations.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\textwidth]{images/Activationsrecur_cnn_8-7-svhn.pdf}
    \caption{Relative activations at each layer in the recurrent module of a residual network trained on CIFAR-10.}
    \label{fig:activations_svhn}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.45\textwidth]{images/Activationsrecur_resnet_19-5.pdf}
    \includegraphics[width=0.45\textwidth]{images/Activationsrecur_resnet_19-6.pdf}\\
    \includegraphics[width=0.45\textwidth]{images/Activationsrecur_resnet_19-9.pdf}
    \includegraphics[width=0.45\textwidth]{images/Activationsrecur_resnet_19-10.pdf}
    \caption{Relative activations at each layer in the recurrent module of a residual network trained on CIFAR-10.}
    \label{fig:activations_resnet}
\end{figure}


\subsection{Classifiability of Features}
\label{sec:app_classify_feats}

Compare the accuracy when a linear classifier is trained on features form different layers. As \citet{kaya2019shallow} do in their study of overthinking, we use average pooling to reduce the size of the features in this experiment.

\begin{table}[h!]
    \begin{center}
    \caption{\textbf{Classifiability of features.} CIFAR-10 classification accuracy of linear classifiers trained on intermediate features output by each residual block (or each iteration) in networks with 19-layer effective depths. Average pooling is used to change the dimension of feature maps in this experiment. This is consistent with \citep{kaya2019shallow}. Each cell reports the percentage of training/testing images correctly labeled.}
    \label{tab:feat_classification_pooled}
    \vspace{5pt}
    \begin{small}
        \begin{tabular}{rcccc}
            \toprule
             & Block \#1 & Block \#2  & Block \#3 & Block \#4 \\
            \midrule
            Feed Forward & 85.7 / 83.4 & 94.1 / 88.0 & 99.4 / 90.2 & 99.8 / 90.8 \\
            Recurrent & 88.1 / 84.1 & 96.9 / 88.4 & 99.7 / 89.8 & 99.9 / 90.4 \\
            \bottomrule
        \end{tabular}
    \end{small}
    \end{center}
\end{table}


\subsection{Feature Visualization}
\label{sec:app_visualization}

We discuss the feature visualization technique we used in \ref{sec:feature_visualization} in further detail. For both ImageNet and CIFAR-10 datasets, we use networks with residual connections.

Similar to \citep{vis_yin2020dreaming}, we use pixel jitter as augmentation and total variation as regularizer. The pixel jitter moves the input image both horizontally and vertically by selecting two random number between $(-32, +32)$ for each axis. The portion of image that moves out of the viewpoint can fill up the empty space on the opposite side. 
For the total variation, we use the anisotropic version in four directions: horizontal, vertical, and two diagonal directions. We use the $\ell_2$-norm for computing the total variation in all directions. 

We find that the batch statistics from the first convolutional layer provides a strong enough signal for improving the quality through regularization.

For CIFAR-10, we optimize a mini-batch of size $n=64$ of $32 \times 32$ images for $1000$ iterations. For ImageNet we use a mini-batch of size $n=32$  of $224\times224$ images for $1000$ iterations. Both experiments are done on a single Nvidia GeForce RTX 2080Ti GPU. 

As the main loss for CIFAR-10 experiments, we maximize the $\ell_2$-norm of activations. More precisely, assuming that $a_{l, f}(x_i)$ represents the activation for filter $f$ in layer $l$ on input $x_i$, then we solve: 
$$ \max_{x} \sum_i \| a_{l,i}(x_i) \|_2$$
For ImageNet experiments, use a contrastive version of the loss to promote diversity:

$$ \max_{x} ( \sum_i n \| a_{l_i}(x_i) \|_2 - \sum_{j \neq i} \| a_{l_i}(x_j) \|_2 ) $$ 

We use the ADAM optimizer and cosine annealing based learning rate schedule. The initial learning rate is $0.01$. 

Assuming that $\lambda_{main}$, $\lambda_{tv}$, $\lambda_{bn}$ represent the coefficients for the main loss, total variation and batch normalization regularizer, respectively, we set $\lambda_{tv}=0$ and $\lambda_{bn}=0$ for the visualizations in the first layer, and linearly increase them as we go deeper. For the last layer, in CIFAR-10 experiments, $\lambda_{main}=0.64$, $\lambda_{tv}=1.0$, and $\lambda_{bn}=10$. For ImageNet experiments, in the deepest layer we set $\lambda_{main}=0.01$, $\lambda_{tv}=5.0$, $\lambda_{bn}=50.0$. 

\subsection{Extensive Qualitative Visualization}
\label{sec:more_visualizations}

Similar to Section \ref{sec:feature_visualization}, here we show the results of our visualizations in Figures \ref{fig:app_visualization_imagenet} and \ref{fig:app_visualization_cifar}.
We note that the first and final layers are not part of the recurrent modules. 

\def \aminlen{0.466\linewidth} 
\begin{figure}
    \centering
        \centering
        \setlength\tabcolsep{0.0pt}
        \begin{tabularx}{\linewidth}{cccc}
            \toprule
                Depth     & Recurrent & ~ & Feed Forward \\
            \hline
            
            1 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/airec0.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/aiffw0.png} }\\ 
            2 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/airec1.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/aiffw1.png} }\\ 
            3 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/airec2.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/aiffw2.png} }\\ 
            4 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/airec3.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/aiffw3.png} }\\ 
            5 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/airec4.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/aiffw4.png} }\\ 
            6 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/airec5.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/aiffw5.png} }\\ 
            7 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/airec6.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/aiffw6.png} }\\ 
            8 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/airec7.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/aiffw7.png} }\\ 
            9 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/airec8.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/aiffw8.png} }\\ 
            10 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/airec9.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/aiffw9.png} }\\ 
            
            \bottomrule
        \end{tabularx}
        \setlength\tabcolsep{6.0pt}
        \caption{ImageNet filter visualization. Filters from recurrent model iterations alongside corresponding feed-forward layers.}
        \label{fig:app_visualization_imagenet}
\end{figure}



\def \aminlen{0.466\linewidth} 
\begin{figure}
    \centering
        \centering
        \setlength\tabcolsep{0.0pt}
        \begin{tabularx}{\linewidth}{cccc}
            \toprule
                Depth     & Recurrent & ~ & Feed Forward \\
            \hline
            
            1 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec0.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw0.png} }\\ 
            2 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec1.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw1.png} }\\ 
            3 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec2.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw2.png} }\\ 
            4 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec3.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw3.png} }\\ 
            5 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec4.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw4.png} }\\ 
            6 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec5.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw5.png} }\\ 
            7 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec6.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw6.png} }\\ 
            8 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec7.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw7.png} }\\ 
            9 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec8.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw8.png} }\\ 
            10 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec9.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw9.png} }\\ 
            11 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec10.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw10.png} }\\ 
            12 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec11.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw11.png} }\\ 
            13 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec12.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw12.png} }\\ 
            14 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec13.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw13.png} }\\ 
            15 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec14.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw14.png} }\\ 
            16 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec15.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw15.png} }\\ 
            17 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec16.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw16.png} }\\ 
            18 & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/cairec17.png}}  & & \raisebox{-0.5\totalheight}{\includegraphics[width=\aminlen]{images/visualization/caiffw17.png} }\\ 
            
            
            
            \bottomrule
        \end{tabularx}
        \setlength\tabcolsep{6.0pt}
        \caption{CIFAR-10 filter visualization. Filters from recurrent model iterations alongside corresponding feed-forward layers.}
        \label{fig:app_visualization_cifar}
\end{figure}
